Measuring the Feasibility of Analogical Transfer using Complexity

Analogies are 4-ary relations of the form "A is to B as C is to D". While focus has been mostly on how to solve an analogy, i.e. how to find correct values of D given A, B and C, less attention has been drawn on whether solving such an analogy was actually feasible. In this paper, we propose a quantification of the transferability of a source case (A and B) to solve a target problem C. This quantification is based on a complexity minimization principle which has been demonstrated to be efficient for solving analogies. We illustrate these notions on morphological analogies and show its connections with machine learning, and in particular with Unsupervised Domain Adaptation.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/related.tex <==
This notion of transferability is interesting to consider in the perspective of task relatedness as defined in Section \ref{subsec:tr:intro:task-relatedness}. The introduced notions are in contrast with the presented measures of task relatedness in the idea that it does not provide a measure of divergence between two distributions in a domain, but between a model (that can be a distribution) and a dataset. Our notion is more general in the sense that it does not rely on any probabilistic setting, and focuses on the description of input data, and not on labels. In this sense, it differs from~\cite{zhang2012generalization}. The choice of not describing the item will be justified below, in a discussion on negative transfer. 

Finally, the difference between our definitions and the divergence introduced by~\cite{mahmud2009universal} is complicated. The first main difference is the purpose. Our approach does not focus on defining a measure of task-relatedness, but to what extent a learned model can be applied to a future problem. Another major difference is the symmetry of the considered divergence, that is not observed in our framework. For us, the order of the task (source or target) plays a role in the notion of relatedness. 

==> sections/transferability-old.tex <==
Analogies involve two separate domains: a \emph{source domain}~$\sourcedom$ and a \emph{target domain}~$\targetdom$. Given a source problem-solution pair $(x^S, y^S) \in \sourcedom$ and a target problem $x^T \in \mathcal{X}^T$, the analogical transfer from $(x^S,y^S)$ to $x^T$ is informally defined as finding $y^T \in \mathcal{Y}^T$ such that the transformation $c \mapsto$ is ``similar" to the transformation $x^S \mapsto y^S$. This notion of similarity is problematic, especially when the source and target domains are distinct. Existing frameworks of analogy often assume that the source and target domains are the same~\cite{MicletPrade}, or at least share a common structure (e.g. are $L$-algebras of a same language~$L$, such as proposed by (Antic, 2020)~\cite{Antic2020}).

In this section, we show how complexity can be used to properly define this similarity, even in the case of distinct domains. We will then show that this definition helps quantifying the notion of \emph{transferability}, i.e. how the source observation $(x^S,y^S)$ is useful to find a solution to target problem~$x^T$. 


\subsection{Inference of a Target Model}

The task in the target domain consists in predicting the solution~$y^T \in \mathcal{Y}^T$ associated to the problem~$x^T \in \mathcal{X}^T$. Usually, this is done throughout a model~$M$, in particular by finding $y^T \in \mathcal{Y}^T$ and $r \in \reprspace$ maximizing the score $M(x^T,y^T,r)$:
\begin{equation}
    y^{T*} \in \text{arg}\max_{y \in \mathcal{Y}^T} \left\lbrace \max_{r \in \mathcal{R}} M(x^T, y, r) \right\rbrace
     \label{eq:model-based-prediction}
\end{equation}
In the context of Example~\ref{ex:morphology-model}, this corresponds to choosing a representation $r$ that successfully describes~$x^T$ given the recursive function~$\phi$ associated to~$M$, i.e. finding $r$ such that $\phi_1(r) = x^T$. The solution~$y^T$ is then estimated by taking $y^T = \phi_2(r)$. In the context of Example~\ref{ex:probabilistic-model}, Equation~\eqref{eq:model-based-prediction} corresponds to taking the most probable solution.  

However, in practice, the model~$M$ is not known and needs to be inferred. The difficulty is that, in general, it is not possible to identify~$M$ given $x^T$ only. Even worse, there is no guarantee that two models correctly describing~$x^T$ can yield the same values of~$y^T$. For instance, in the morphological domain (Example~\ref{ex:morphology-model}), one can build degenerate functions~$\phi$ such that $\phi(r) = x^T$ for all $r$. All such functions successfully describe~$x^T$ and yield all possible values for~$ y^T$. 

Such as for the inference on the source domain, we propose to rely on the MML principle to estimate the target model $M$. However, in the context of an analogy, some additional information is provided by the observation of the source domain, where a model~$M^S$ can be evaluated from observations~$(x^S, y^S) \in \sourcedom$. The target model~$M^T$ can then be described with regards to the source model~$M^S$. 

The limitation of such a relative description of models is that the source model may not be relevant. In the following, we propose to quantify this relevance with two measures of model reusability, 



\subsection{Reusability of a Source Model}

We measure the reusability of a source model to its ability to compress the information about the target domain. We identify two main possible definitions, that we call \emph{weak} and \emph{strong} reusability, and will show that a strongly reusable model is necessarily weakly reusable. 

The main criterion for \emph{weak reusability} is that knowing the source model~$M^S$ makes the target inference better, in the sense that it compresses more the description of the target problem~$x^T$. 
 
\begin{definition}[Weak reusability]
Let $\eta > 0$.
A model~$M^S \in \mathbb{M}_{\mathcal{R}^S, \dom^S}$ is called \emph{weakly $\eta$-reusable} for problem $x^T$ in target model space~$\mathbb{M}_{\mathcal{R}^T, \dom^T}$ if:
\begin{align}
\min_{M \in \mathbb{M}_{\mathcal{R}^T, \dom^T}} \lbrace & K(M) + K(x^T | M) \rbrace \nonumber \\
& \geq \min_{M \in \mathbb{M}_{\mathcal{R}^T, \dom^T}} \lbrace K(M | M^S) + K(x^T | M) + \eta \rbrace \label{eq::weak-reusability}
\end{align}
\label{def:weak-reusability}
\end{definition}

It is essential to keep in mind that this definition is relative to the choice of a model space~$\mathbb{M}_{\mathcal{R}^T, \dom^T}$ for the target domain. A source model~$M^S$ may not be reusable for a problem $x^T$ depending on the chosen target model space. In the following, we will abusively omit to mention the target model space, for readability purposes. 

Note that the models~$M$ defined in the left-hand side and in the right-hand side of inequality~\eqref{eq::weak-reusability} are not the same. On the left-hand-side, the model corresponds to the optimal target model describing~$x^T$ while, on the right-hand-side, it is the optimal model describing~$x^T$ when $M^S$ is known. 

This notion of reusability means that providing the source model~$M_S$ helps finding a new description of the problem shorter than the optimal description by~$\eta$ bits. 
In particular, in the case where $\mathbb{M}_{\mathcal{R}^S, \dom^S} = \mathbb{M}_{\mathcal{R}^T, \dom^T}$, the optimal model for $x^T$ (i.e. the model that minimizes $K(M) + K(x^T|M)$) is trivially weakly reusable for $x_T$. In other words, when the optimal model for the source domain is also optimal for the target domain, then it is obviously reusable for the target domain. The interesting case will be when the optimal source model is not optimal for the target domain. 

We notice that the definition does not require $\sourcedom = \targetdom$ and aims to quantify the reusability of a model even for a completely different task. This is possible since complexity only requires to have computable models: Indeed, the term $K(M | M^S)$ is defined as long as the models are computable. 
In practice, the issue of comparing objects of different nature is hidden within the choice of the reference p.r.p. function for complexity (see Section~\ref{sec:kolmogorov}). 

\medskip

We propose an alternative definition of reusability, called \emph{strong reusability}. 
It is based on the idea that $M_S$ is reuseable if it helps compressing the optimal model of target problem~$x^T$. Unlike previous definition, $M_S$ is not directly involved in the description of~$x^T$ though. 

\begin{definition}[Strong reusability]
Let $\eta > 0$.
A model~$M^S \in \mathbb{M}_{\mathcal{R}^S, \dom^S}$ is called \emph{strongly $\eta$-reusable} for problem $x^T$ in target model space~$\mathbb{M}_{\mathcal{R}^T, \dom^T}$ if:
\begin{align}
M \in \underset{M \in \mathbb{M}_{\mathcal{R}^T, \dom^T}}{\text{arg} \min} \lbrace & K(M) + K(x^T | M) \rbrace \nonumber \\
& \Longrightarrow K(M) \geq K(M | M^S) + \eta \label{eq:strong-reusability}
\end{align}

\label{def:strong-reusability}
\end{definition}

This definition also relies on the choice of a target model space. As for weak reusability, we will abusively omit the model space in the following notations. 

Strong reusability is an extremely strong property of a source model. Indeed, it would be a natural property that, in case~$\mathbb{M}_{\mathcal{R}^S, \dom^S} = \mathbb{M}_{\mathcal{R}^T, \dom^T}$, any model minimizing $K(M) + K(x^T | M)$ is reusable to~$x^T$. This is not the case for strong reusability: indeed, the definition implies that \emph{any} model minimizing $K(M) + K(x^T | M)$ can be compressed given $M^S$, not only $M^S$ itself. Note that this could be alleviated by weakening Definition~\ref{def:strong-reusability} and requiring only the existence of a model $M$ minimizing $K(M) + K(x^T | M)$ and such that $K(M) \geq K(M | M^S) + \eta$. 




\subsection{Properties of Reusability}

We now present basic properties of these two notions of reusability. All the presented properties follow directly from the definitions. 


The first property applies to both weakly and strongly reusable models: it states that the threshold~$\eta$ is not unique. The proof of this proposition is trivial and omitted. 

\begin{proposition}
Let~$M_S \in \mathbb{M}_{\mathcal{R}^S, \dom^S}$ and $x^T \in \mathcal{X}^T$. If $M^S$ is $\eta$-reusable for $x^T$, then it is also $\eta^\prime$-reusable for $x^T$ for all $\eta^\prime \leq \eta$.
In the following, we will call \emph{degree of reusability} of $M^S$ to $x^T$ the quantity:
\begin{equation}
    \rho(M^S, x^T) = \max \left\lbrace \eta \  ; \ M^S \text{ is } \eta \text{-reusable for } x^T \right\rbrace
    \label{eq:degree-reusability}
\end{equation}
\label{prop:reusability-monotonicity}
\end{proposition}

However, we insist on the fact that the degree of reusability is relative to a chosen target model space. It also depends on which of weak or strong reusability is considered. 
This dependency would not exist if these two notions of resuability were equivalent, which we will see is not the case. We will use the notation $\rho_w$ and $\rho_s$ to specify between the weak and strong cases. 


We now show that strong reusability implies weak reusability: 

\begin{proposition}
Let $M^S \in \mathbb{M}_{\mathcal{R}^S, \dom^S}$ a source problem, a target problem $x^T \in \mathcal{X}^T$ and $\eta > 0$.
If $M^S$ is strongly $\eta$-reusable for $x^T$, then $M^S$ is also weakly $\eta$-reusable for $x^T$. 
\label{prop:correlation-reusability}
\end{proposition}

\begin{proof}
We call~$M^* \in \mathbb{M}_{\mathcal{R}^T, \dom^T}$ an optimal model for $x^T$: $M^* \in \text{arg} \min_M \lbrace K(M) + K(x^T | M) \rbrace$. 
Under the assumptions of the proposition, it follows that:
\begin{align*}
\min_M \lbrace &K(M) + K(x^T | M) \rbrace \\
& = K(M^*) + K(x^T | M^*) \\
&\geq K(M^* | M^S) + \eta + K(x^T | M^*) \\
&\geq \min_M \lbrace K(M | M^S) + K(x^T | M) + \eta \rbrace
\end{align*}
which proves the proposition.
\end{proof}

However, the converse is not true: weak reusability does not imply strong reusability. This is the consequence of the fact that the models implied in Equation~\eqref{eq::weak-reusability} are not the same on the right hand side and on the left-hand side. We illustrate this with a simple example.

\begin{example}
\label{ex:weak-notstrong}
We consider a target model space made up of two distinct models: $\mathbb{M}_{\mathcal{R}^T, \dom^T} = \lbrace M_1, M_2 \rbrace$. We assume the following properties:
\begin{itemize}
    \item $M_1$ and $M_2$ describe equally well problem~$x^T$, in the sense that $K(x^T | M_1) = K(x^T | M_2)$
    \item Model $M_1$ is more complex than model~$M_2$: $K(M_1) > K(M_2)$
    \item Model $M_1$ is easily described by source model~$M^S$: for simplicity, we can take~$K(M_1 | M^S) = 0$
    \item Model $M_2$ is not well described by source model~$M^S$: for simplicity, we can take~$K(M_2 | M^S) = K(M_2)$
\end{itemize}

With these assumptions, it can be easily verified that $M^S$ is weakly $\eta$-reusable for~$x^T$, with $\eta \leq K(M_2)$. However, $M^S$ is not strongly $\eta$-reusable for~$x^T$, since $M_2$ minimizes $K(M) + K(x^T | M)$ but $K(M_2) < K(M_2) + \eta = K(M_2 | M^S) + \eta$. 

\end{example}


Putting together the results of Propositions~\ref{prop:reusability-monotonicity} and \ref{prop:correlation-reusability}, as well as the counter-example of Example~\ref{ex:weak-notstrong}, we can establish the following result:
\begin{corollary}
For~$M_S \in \mathbb{M}_{\mathcal{R}^S, \dom^S}$ and $x^T \in \mathcal{X}^T$:
\begin{equation}
    \rho_s(M^S, x^T) \leq \rho_w(M^S, x^T)
\end{equation}
\end{corollary}






\subsection{Transferable Cases}

The notion of  reusability we proposed in Definitions~\ref{def:weak-reusability} and~\ref{def:strong-reusability} are not directly applicable to measure transferability from a source observation to a target problem. The property of transferability measures the ability to transfer knowledge from a solved problem~$(x_S, y_S) \in \sourcedom$ to apply it on the unsolved target problem~$x^T \in \mathcal{X}^T$. It can be seen as an extension of reusability where the source model~$M^S$ is determined based on the source observation. 

\begin{definition}[Transferability]
\label{def:transferability}
Let $(x^S, y^S) \in \sourcedom$ be a source case. The case~$(x^S, y^S)$ is said to be strongly (resp. weakly) $\eta$-transferable to the problem~$x^T \in \mathcal{X}^T$ if the set of compatible models $\lbrace M^S | K(M^S) + K(x^S, y^S | M_S) < K(x^S, y^S), M^S \in \mathbb{M}_{\mathcal{R}^S, \dom^S} \rbrace$ contains an element $M^{S*}$ such that $M^{S*}$ is strongly (resp. weakly) reusable for problem~$x^T$. 
\end{definition}

The proposed definition of transferability is very weak, since it only requires the existence of one source model that is reusable. However, it does not take into account the quality of this model in the source domain. For instance, it would acquire equal weight if the reusable source model is associated with complexity $K(M^S) + K(x^S, y^S | M^S)$ close to $K(x^S, y^S)$, as if the complexity is close to 0. Such situations are very likely to occur with probabilistic models, since many such models give positive probability to all observations.

In order to refine this notion, it would be important to define a coefficient of transferability, similar to the degree of reusability~$\rho$ defined in Proposition~\ref{prop:reusability-monotonicity}. We will denote such a coefficient $\tau((x^S, y^S), x^T)$. We propose twp possible definitions below. These definitions rely on the set of compatible models for $(x^S, y^S)$ introduced in Definition~\ref{def:transferability}, and denoted~$\mathbb{M}(x^S, y^S)$. 

A first definition is a direct application of Definition~\ref{def:transferability}: it associates the transferability of a problem to the maximum reusability of the corresponding model:
\begin{equation}
\tau_{\text{max}}\left((x^S, y^S), x^T\right) = \max_{M^S \in \mathbb{M}(x^S, y^S)} \rho(M^S, x^T) 
\label{eq:transferability-max}
\end{equation}
with the convention that $\max \emptyset = 0$. 
This definition has the same weakness as the introduced concept of transferability: it does not take into account that the most reusable model might also be very weak to describe $(x^S, y^S)$. 

In order to alleviate this, our second definition propose to average the score over the possible models. Therefore, we compute the posterior of the model for given~$(x^S, y^S)$ and compute the score as the expected value over~$M_S$ of the degree of reusability. 
\begin{equation}
\tau_{\text{avg}}\left((x^S, y^S), x^T\right) = \sum_{M^S \in \mathbb{M}(x^S, y^S)} p(M^S | x^S, y^S) \rho(M^S, x^T) 
\label{eq:transferability-avg}
\end{equation}
In order to compute the posterior~$p(M^S | x^S, y^S)$, we use algorithmic probability~\cite{li2008introduction} and assume a uniform prior:
\begin{equation}
    p(M^S | x^S, y^S) = 2^{- K(x^S, y^S | M^S) - K(M^S)}
\end{equation}
This second definition provides a better idea of how transferable a source observation can be, since it takes into account all possible models describing it. However, it has two major weaknesses. On a theoretical level, it does not does not reflect the variance of the reusability degree over the compatible models: based on $\rho_{\text{avg}}$ only, it is impossible to know whether all models, only very few but very compatible models, or a large number of less compatibles are reusable. On a practical level, the $\tau_{\text{avg}}$ score may not be tractable, and would require some approximations. 



\subsection{Non-Transferability and Negative Transfer}

The notion of \emph{negative transfer}~\cite{wang2019characterizing} is inherent to any form of transfer, while going against the intuition that more information necessarily brings better performance. Negative transfer designates a situation where the source problem brings \emph{negative} information to the resolution of the target problem.

Although tempting, it would be incorrect to assimilate negative transfer to non-transferability. On the contrary, negative transfer occurs when transfer is possible ($\rho > 0$) but leads to incorrect results. In the transfer scenario considered in this paper, the major cause for negative transfer is the fact that only the distribution over~$\mathcal{X}^T$ is known, and taken into account both in the target inference (Equation~\eqref{eq:model-based-prediction}) and in the definitions of reusability (Definitions~\ref{def:weak-reusability} and \ref{eq:strong-reusability}) and of transferability (Equations~\eqref{eq:transferability-max} and \eqref{eq:transferability-avg}). 



